Development and Adaptation of Robotic Vision in the Real-World: the Challenge of Door Detection

Mobile service robots are increasingly prevalent in human-centric, real-world domains, operating autonomously in unconstrained indoor environments. In such a context, robotic vision plays a central role in enabling service robots to perceive high-level environmental features from visual observations. Despite the data-driven approaches based on deep learning push the boundaries of vision systems, applying these techniques to real-world robotic scenarios presents unique methodological challenges. Traditional models fail to represent the challenging perception constraints typical of service robots and must be adapted for the specific environment where robots finally operate. We propose a method leveraging photorealistic simulations that balances data quality and acquisition costs for synthesizing visual datasets from the robot perspective used to train deep architectures. Then, we show the benefits in qualifying a general detector for the target domain in which the robot is deployed, showing also the trade-off between the effort for obtaining new examples from such a setting and the performance gain. In our extensive experimental campaign, we focus on the door detection task (namely recognizing the presence and the traversability of doorways) that, in dynamic settings, is useful to infer the topology of the map. Our findings are validated in a real-world robot deployment, comparing prominent deep-learning models and demonstrating the effectiveness of our approach in practical settings.

==> contents/01-introduction-old.tex <==
\section{Introduction}\label{sec:intro}
\red{OLD INTRO}
Mobile service robots represent a flourishing technology increasingly employed across a range of human--centric, real--world domains such as office and domestic environments. Typically deployed for the long term, these robots find in \emph{robotic vision} -- the ability to understand semantic knowledge from visual robot perceptions in real time-- a cornerstone to achieving high--level autonomy and operational awareness. Indeed, one of the key capabilities is the one to detect objects, which can significantly enhance a variety of sub--tasks across increasing levels of abstraction, including localization, navigation, scene understanding, and planning.

Recent developments in object detection, largely driven by research in deep learning, have unlocked remarkable possibilities for addressing this real--world AI challenge, facilitating the creation of highly effective vision modules for mobile robots. However, despite the abundance and diversity of available models, their practical application in field robotics continues to pose methodological and practical challenges. In this work, we introduce a method designed to address them in the context of a particularly significant task for service robots, whose functionalities are strongly based on autonomous navigation: \emph{door detection}. 

Doors are key environmental features for a mobile robot. They represent the topological connections between adjacent sub--regions of the free space whose traversability, importantly, might not always be possible. 
%More specifically, our definition of a door is centered on the notion of variable--traversability passage, without necessarily assuming the presence of typical door components like a leaf, a hinge, or any other related furniture (this is what in the literature is commonly referred to as ``explicit'' doors~\cite{whiting2007topology}). 
\revI{For this reason, in this work address the typical operational requirements of indoor service robots by defining a door as a variable--traversability passage.
This approach is broader and hence more complex than adopting the more conventional concept of ``explicit'' door (as defined in~\cite{whiting2007topology}), which is based physical structures with components like a leaf, a hinge, or any other related furniture.}
Door detection is the capability for a robot to recognize in real--time the location and traversability status (\texttt{open} or \texttt{closed}) of such passages. This problem is most effectively addressed as an object detection task using RGB images acquired by the robot, primarily due to the limitations of alternative technologies. For example, laser range scanners, while excellent for distance measurements, are typically constrained by a 2D field of view. In the same line, \mbox{RGB--D} cameras often exhibit a limited depth sensing range, making them less reliable over longer distances or in larger indoor spaces. Furthermore, both types of sensors can struggle with transparent or highly reflective surfaces, that are often present in doors. Figure~\ref{fig:giraff} illustrates the execution of door detection: a mobile robot navigates in an environment to perform its tasks; at the same time it acquires images through its onboard camera. For each image, it infers in real--time the bounding boxes of doors, distinguishing between open doors (depicted in green) and closed ones (depicted in red), also highlighted on the map. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\linewidth]{images/fig1.png}
\caption{Giraff--X~\cite{GIRAFF}, the service robot adopted in this work, performing door detection.}
\label{fig:giraff}
\end{figure}

In practical deployments, service robots are subject to specific perception constraints and frequently encounter challenging recognition instances, such as partially occluded or poorly positioned viewpoints. These challenges are intrinsic to the domain of service robots, as they are designed to operate in environments marked by dynamism and clutter. This condition induces critical domain shifts over the state--of--the--art object detectors, which are typically trained over datasets that largely neglect the noisy, constrained, and challenging operational conditions that a robot faces on the field. Properly and efficiently adapting these models for service robots is an open methodological problem, yet one of remarkable practical importance.

Two important facts should be considered about a robot operating in its target environment: on one side, human--centric indoor environments are indeed complex and difficult to process using computer vision due to the aforementioned challenges. On the other side, while the position of the objects in the target environment is highly dynamic, the robot will see the same object instances multiple times. Moreover, different instances of the same type of object will likely have a similar aspect. For example, while it is highly likely that two chairs from two different environments look very different, the chairs around the same table are usually of the same model. The same holds for doors. As a result of this, the robot during its daily activities will observe multiple times the same set of objects, and sets of objects similar among them. This fact can be used to improve the perceptual capabilities of the robot in its target environment, compensating for the challenges of the domain.

In this work, we demonstrate how the integration of simulation frameworks and domain adaptation techniques can create an effective development pipeline for constructing door detectors specifically tailored for mobile service robots.  Specifically, the contributions we provide are the following. 

\begin{itemize}
\item We analyze the trade--offs involved in using simulations to train a door detector capable of generalizing effectively across various environments. We delineate the desiderata of this process and propose a framework based on simulation performed in 3D real--world models, Gibson~\cite{gibson}, that achieves a balance between data photorealism and acquisition costs.
\item We explore fine--tuning to qualify detectors to a robot's target environment, demonstrating how leveraging typical operational settings of service robots can enhance performance in challenging instances.
\item We argue that performance metrics used to evaluate computer--vision models are not well suited to be used in a robotic context, and we propose new evaluation metrics specifically designed to better reflect our setting.
%\item We conduct an extensive experimental campaign with three prominent deep--learning models for object detection, providing insights into how domain shifts in our scenario are influenced by the nature of the training datasets.
\item We conduct an extensive experimental campaign with three \revI{state--of--the--art and widely adopted} deep--learning models for object detection, providing insights into how domain shifts in our scenario are influenced by the nature of the training datasets.
\item We assess them on both general and environment--specific door detectors, identifying the most effective training setups.  We evaluate the trade--off between training efforts and performance improvements, validating our findings in an actual deployment on a service robot.
\item We evaluate the impact of different performance of a door detection method on a downstream task, that is to evaluate the current traversability status of the whole environment.
\end{itemize}

%% Paper summary
In the next section, we briefly survey the related works relevant to this study. Section~\ref{sec:method} motivates and outlines our methods while the remainder of the paper is devoted to experimental analysis. Section~\ref{sec:evaluation} extensively analyses the performance of our general and qualified detectors while Section~\ref{sec:onTheFieldExp} focuses on the evaluation in a real robot deployment. Concluding remarks are provided in Section~\ref{sec:conclusions}.

The contributions of this paper build upon and extend our earlier work presented in~\cite{antonazzi2023enhancing}, where we have illustrated a preliminary version of the findings presented here. In this work, we significantly extend the experimental evaluation also by assessing multiple models for object detection.

%% old schema
\begin{comment}
\begin{itemize}
\item Motivating scenario: autonomous service robots are deployed in a variety of real-world environments. They are a promising technology. They cover many different tasks, examples can be found in assistance, logistics, and surveillance. They typically operate in the same environment for a long time.
\item Many tasks performed by service robots depend on their ability to autonomously construct models of the environment and make inferences from them. Achieving this capability requires the extraction of high-level knowledge from real-world perceptions. For instance, this includes tasks like creating a map and performing navigation on it in order to accomplish specific tasks.
\item In this paper, we focus on one of these challenges that service robots must address, which is the real-time recognition of environmental features using RGB cameras, a.k.a. Robotic Vision.
\item Why are we considering this task? For two reasons.  
\begin{enumerate}
    \item Significance. The ability to recognize visual features within the environment plays a key role in enhancing a service robot's operational awareness. This, in turn, holds the potential to improve tasks such as localization, navigation, semantic understanding, and planning. These aspects collectively underpin the effectiveness of service robot deployments, making this challenge very important.
    \item Hardness profile. This task offers a relatively low entry barrier, meaning that achieving a baseline level of performance is attainable without much effort (a great deal here is played by the availability of off-the-shelf detectors). However, it also presents an intriguing high ceiling. In practical deployments, service robots frequently encounter challenging recognition instances, such as identifying partially occluded objects or contending with poorly positioned viewing angles. These challenges are intrinsic to the domain of service robots, as they are typically subject to perception constraints in environments marked by dynamism and clutter. The development of detectors capable of consistently delivering high-quality performance under such conditions is quite hard. Importantly, these difficult instances can have a great impact on the service provided by the robot.
\end{enumerate}
\item How is this task addressed today? The family of techniques is that of deployed/applied Computer Vision. In our work we shall call it Robotic Vision, to make explicit its grounding to our robotic domain. \textit{[Provide many references to underline that Deployed/Applied/Robotic Vision, and not just CV, is a research area with its own challenges]} Early techniques were based on manually defined features, today the arena is dominated by deep-learning detectors which have been trained to localize a variety of object classes in RGB images. These detectors are typically trained on large datasets of images taken from a wide range of viewpoints and angles (for example, COCO~\cite{coco}). Such a variety of viewpoints does not represent in any way the typical robot POV.
\item Research question: how to build and deploy robotic vision modules in service robots?
\item Why is the research question important? From one side there are many readily available deep-learning Computer Vision (CV) models and architectures. However, naively deploying those models simply does not work, for a number of reasons that, in this paper, we empirically show and discuss. A general methodology for this challenge is still far from being accepted and well-defined. Contributing to it (like we do in our paper) will allow practitioners to better leverage the potential of deep-learning CV models in service robots.
\item What's our original contribution? We contribute to a methodology to deploy deep robotic vision on service robots. Our proposed methodology is made by two steps.
\begin{enumerate}
    \item Building a \emph{General Detector} (GD). 
    This is an object detector that can deliver consistent performance across diverse operational environments, which is why we refer to it as ``general''. We demonstrate the limitations of adopting bare off-the-shelf detectors and emphasize the need for re-training using image acquisitions that properly represent the robot's POV. We discuss a tradeoff between training costs and achieved performance, proposing a method based on simulation that can balance the two factors in a satisfactory way. We show that this technique is valid and achieves acceptable performance in the real world.   
    \item Obtaining a \emph{Qualified Detector} (QD). This is a detector that has been specialized (fine-tuned) for the specific environment in which the robot has to operate. We exploit some features of our reference scenario (the fact that there's an initial installation phase to which a long operation time follows) to perform fine-tuning with additional data gathered in the target environment. We empirically evaluate the costs of this procedure comparing them with the obtained benefits. We show that the method is valid and achieves good performance in difficult instances encountered in the real world.
\end{enumerate}
We extensively evaluate our method in two real indoor use cases for service robots.
\begin{enumerate}
    \item Detection of passages between rooms. This is a task that has a remarkable impact on navigation tasks in an environment where the connectivity between areas can vary.
    \item Detection of landmarks. This is a key task that can boost localization. \textcolor{red}{Consider removing.}
\end{enumerate}
\end{itemize}
\end{comment}



==> graphics/legend_ap_qualified_detector.tex <==
\addlegendimage{ybar,area legend,draw=steelblue31119180,fill=steelblue31119180}
\addlegendentry{$GD$}
\addlegendimage{ybar,area legend,draw=darkorange25512714,fill=darkorange25512714,opacity=0.9,thick}
\addlegendentry{$QD_{e}^{15}$}
\addlegendimage{ybar,area legend,draw=black,fill=none,opacity=0.9,thick,postaction={pattern=north east lines, fill opacity=0.9}}
\addlegendentry{Closed door}
\addlegendimage{ybar,area legend,draw=forestgreen4416044,fill=forestgreen4416044,opacity=0.9,thick}
\addlegendentry{$QD_{e}^{25}$}
\addlegendimage{ybar,area legend,draw=crimson2143940,fill=crimson2143940,opacity=0.9,thick}
\addlegendentry{$QD_{e}^{50}$}
\addlegendimage{ybar,area legend,draw=black,fill=none,opacity=0.9,thick}
\addlegendentry{Open door}

==> graphics/legend_comparison_extended_metric.tex <==
\addlegendimage{forestgreen4416044,mark=*,mark size=3}
\addlegendentry{$TP_{\%}$}
\addlegendimage{darkorange25512714,mark=diamond*,mark size=3}
\addlegendentry{$BFD_{\%}$}
\addlegendimage{crimson2143940,mark=triangle*,mark size=3}
\addlegendentry{$FP_{\%}$}

==> graphics/legend_comparison_map.tex <==
\addlegendimage{ybar,area legend,draw=forestgreen4416044,fill=forestgreen4416044}
\addlegendentry{DETR~\cite{detr}}
\addlegendimage{ybar,area legend,draw=darkorange25512714,fill=darkorange25512714,opacity=0.9,thick}
\addlegendentry{YOLOv5~\cite{yolov5}}
\addlegendimage{ybar,area legend,draw=crimson2143940,fill=crimson2143940,opacity=0.9,thick}
\addlegendentry{Faster R--CNN~\cite{fasterrcnn}}
\addlegendimage{ybar,area legend,draw=black,fill=none,opacity=0.9,thick,postaction={pattern=north east lines, fill opacity=0.9}}
\addlegendentry{Closed door}
\addlegendimage{ybar,area legend,draw=black,fill=none,opacity=0.9,thick}
\addlegendentry{Open door}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/table_dowstream_task.tex <==
\begin{table}[tb]
\setlength\tabcolsep{4.5pt}
\setlength\extrarowheight{2pt}
\centering
\begin{scriptsize}
\begin{tabular}{cc|ccccc}
\toprule
        \textbf{Env.} & \textbf{Exp.} & \greensquare{} \redsquare{} $\uparrow$ & \greencross{} \redcross{} $\downarrow$ & \yellowcross{} $\downarrow$ &  \graycross{} $\downarrow$ & $RA$ $\uparrow$ \\
\midrule
\multirow{2}{*}{$e_1$} & $GD$ & 20 & 4 & 1 & 2 & 71\% \\
& $QD_e^{15}$ & 25 & 1 & 1 & 1 & 89\% \\[2pt]\hline
\multirow{2}{*}{$e_2$} & $GD$ & 26 & 9 & 4 & 3 & 62\% \\
& $QD_e^{15}$ & 40 & 1 & 1 & 0 & 95\% \\
\bottomrule
\end{tabular}
\end{scriptsize}
\caption{Performance of the downstream task in $e_1$ and $e_2$ obtained using YOLOv5 detectors based in our dataset \DG.}
\label{tab:dowstream_task}
\end{table}
